Progressive Material Caching

The evaluation of material networks is a relatively resource-intensive process in the rendering pipeline. Modern production scenes can contain hundreds or thousands of complex materials with massive networks, so there is a great demand for an efficient way of handling material networks. In this paper, we introduce an efficient method for progressively caching the material nodes without an overhead on the rendering performance. We evaluate the material networks as usual in the rendering process. Then, the output value of part of the network is stored in a cache and can be used in the evaluation of the next materials. Using our method, we can render the scene with performance equal to or better than that of the method without caching, with a slight difference in the images rendered with caching and without it.

==> algorithm/updateAlg.tex <==
% \normalem % disable auto underline

\begin{algorithm}[t]
\caption{Update of a hash table on the GPU}
\label{alg:update}
\SetKwInOut{Input}{Input}
\SetKwFunction{Hash}{Hash}
\SetKwFunction{HashSec}{Hash2}
\SetKwFunction{Encode}{Encode}
\SetKwFunction{CAS}{CAS}

\SetKwFunction{FUpdate}{UpdateHashTable}
\SetKwProg{Fn}{Function}{:}{}

\KwIn{Descriptor of the cacheable node $desc$, the cacheable node's value $v$, array of material cache $matCache$, the number of cells $N_c$ and the number of entries $N_e$.}
\BlankLine
\Fn{\FUpdate{$desc$, $v$, $matCache$, $N_c$, $N_e$}}{
$cellIdx \gets \Hash{desc} \% N_c$\;
$hashVal \gets \HashSec{desc}$\;
$hashIdx \gets -1$\;
\For{$i \leftarrow 0$ \KwTo $N_e$}
{
    $entryIdx \gets cellIdx \times N_e + i$\;
    $current \gets matCache[entryIdx]$\;
    \If{$current.hash = hashVal \cup current.hash = 0$}{
        $hashIdx \gets entryIdx$\;
        $break$\;
    }
}
\If{$hashIdx \neq -1$}
{
    $encodedVal \gets \Encode{v}$\;
    $new \gets \{hashVal,encodedVal\}$\;
    $old \gets \CAS{matCache[hashIdx], 0, new}$\;
}

}
\end{algorithm}

\begin{algorithm}[t]
\caption{Evaluation of the material graph}
\label{alg:update2}
\SetKwFunction{FUpdate}{UpdateHashTable}
\SetKwFunction{MipUv}{CalcVirtualMipmappedTex}

\KwData{array of material cache $matCache$, the number of cells $N_c$, the number of entries $N_e$ and the texture-coordinate gradients $\vec{g_1}$ and $\vec{g_2}$}
\BlankLine

\While{Material graph has a node}{
\Switch{nodeType}{
    \Case{Cache Lookup Node}
    {
        \If{Found the cacheable node in the cache}
        {
            $v \gets cachedVal$\;
            skip the sub-graph under the cacheable node\;
            go to next node of the cacheable node\;
        }
    }
    \Case{Cache Store Node}
    {
        \If{Sub-graph has UV-dependent nodes}
        {
            $(mipLevel, texIndices) \gets$ \MipUv{uv, $\vec{g_1}$, $\vec{g_2}$}\;
        }
        $desc \gets \{matIdx,nodeIdx,mipLevel,texIndices\}$\;
        \FUpdate{$desc$, $v$, $matCache$, $N_c$, $N_e$}
    }
    \Other
    {
        Manage the material node in the standard way\;
        $v \gets nodeVal$\;
    }
}
go to next node\;
}

\end{algorithm}

% \ULforem % enable auto underline
